Application of Random Matrix Theory in High-Dimensional Statistics

This review article provides an overview of random matrix theory (RMT) with a focus on its growing impact on the formulation and inference of statistical models and methodologies. Emphasizing applications within high-dimensional statistics, we explore key theoretical results from RMT and their role in addressing challenges associated with high-dimensional data. The discussion highlights how advances in RMT have significantly influenced the development of statistical methods, particularly in areas such as covariance matrix inference, principal component analysis (PCA), signal processing, and changepoint detection, demonstrating the close interplay between theory and practice in modern high-dimensional statistical inference.

==> custom.tex <==
@article{wishart1928generalised,
  title={The generalised product moment distribution in samples from a normal multivariate population},
  author={Wishart, John},
  journal={Biometrika},
  pages={32--52},
  year={1928},
  publisher={JSTOR}
}


@book{mardia2024multivariate,
  title={Multivariate analysis},
  author={Mardia, Kanti V and Kent, John T and Taylor, Charles C},
  volume={88},
  year={2024},
  publisher={John Wiley \& Sons}
}


@book{muirhead2009aspects,
  title={Aspects of multivariate statistical theory},
  author={Muirhead, Robb J},
  year={2009},
  publisher={John Wiley \& Sons}
}


@article{tulino2004random,
  title={Random matrix theory and wireless communications},
  author={Tulino, Antonia M and Verd{\'u}, Sergio and others},
  journal={Foundations and Trends{\textregistered} in Communications and Information Theory},
  volume={1},
  number={1},
  pages={1--182},
  year={2004},
  publisher={Now Publishers, Inc.}
}

@book{couillet2022random,
  title={Random matrix methods for machine learning},
  author={Couillet, Romain and Liao, Zhenyu},
  year={2022},
  publisher={Cambridge University Press}
}


@article{james2014concise,
  title={Concise probability distributions of eigenvalues of real-valued Wishart matrices},
  author={James, Oliver and Lee, Heung-No},
  journal={arXiv preprint arXiv:1402.6757},
  year={2014}
}


@article{marchenko1967distribution,
  title={Distribution of eigenvalues for some sets of random matrices},
  author={Marchenko, Vladimir Alexandrovich and Pastur, Leonid Andreevich},
  journal={Matematicheskii Sbornik},
  volume={114},
  number={4},
  pages={507--536},
  year={1967},
  publisher={Russian Academy of Sciences, Steklov Mathematical Institute of Russian~…}
}

@article{bai1988convergence,
  title={Convergence to the semicircle law},
  author={Bai, Zhidong D and Yin, Yong Q},
  journal={The Annals of Probability},
  volume={16},
  number={2},
  pages={863--875},
  year={1988},
  publisher={Institute of Mathematical Statistics}
}

@article{yin1987limit,
  title={Limit Theorems for the Eigenvalues of a Product of Large Dimensional Random Matrices When the Underlying Distribution is Isotropic},
  author={Yin, Yong-Quan and Krishnaiah, Paruchuri Rama},
  journal={Theory of Probability \& Its Applications},
  volume={31},
  number={2},
  pages={342--346},
  year={1987},
  publisher={SIAM}
}

@article{hui2010limiting,
  title={Limiting spectral distribution for large sample covariance matrices with m-dependent elements},
  author={Hui, Jun and Pan, Guangming},
  journal={Communications in Statistics—Theory and Methods},
  volume={39},
  number={6},
  pages={935--941},
  year={2010},
  publisher={Taylor \& Francis}
}

@article{wei2016limiting,
  title={The limiting spectral distribution for large sample covariance matrices with unbounded m-dependent entries},
  author={Wei, Meng and Yang, Guangyu and Yang, Lingling},
  journal={Communications in Statistics-Theory and Methods},
  volume={45},
  number={22},
  pages={6651--6662},
  year={2016},
  publisher={Taylor \& Francis}
}

@article{hofmann2008wigner,
  title={Wigner theorems for random matrices with dependent entries: ensembles associated to symmetric spaces and sample covariance matrices},
  author={Hofmann-Credner, Katrin and Stolz, Michael},
  year={2008}
}

@article{friesen2013gaussian,
  title={Gaussian fluctuations for sample covariance matrices with dependent data},
  author={Friesen, Olga and L{\"o}we, Matthias and Stolz, Michael},
  journal={Journal of Multivariate Analysis},
  volume={114},
  pages={270--287},
  year={2013},
  publisher={Elsevier}
}


@article{gotze2006limit,
  title={Limit theorems for spectra of positive random matrices under dependence},
  author={Gotze, F and Tikhomirov, A},
  journal={Journal of Mathematical Sciences},
  volume={133},
  pages={1257--1276},
  year={2006},
  publisher={Springer}
}

@article{yao2012note,
  title={A note on a Mar{\v{c}}enko--Pastur type theorem for time series},
  author={Yao, Jianfeng},
  journal={Statistics \& probability letters},
  volume={82},
  number={1},
  pages={22--28},
  year={2012},
  publisher={Elsevier}
}

@article{silverstein1995strong,
  title={Strong convergence of the empirical distribution of eigenvalues of large dimensional random matrices},
  author={Silverstein, Jack W},
  journal={Journal of Multivariate Analysis},
  volume={55},
  number={2},
  pages={331--339},
  year={1995},
  publisher={Elsevier}
}

@article{bao2012strong,
  title={Strong convergence of ESD for the generalized sample covariance matrices when p/n→ 0},
  author={Bao, Zhigang},
  journal={Statistics \& Probability Letters},
  volume={82},
  number={5},
  pages={894--901},
  year={2012},
  publisher={Elsevier}
}


@book{billingsley2013convergence,
  title={Convergence of probability measures},
  author={Billingsley, Patrick},
  year={2013},
  publisher={John Wiley \& Sons}
}

@article{paul2014random,
  title={Random matrix theory in statistics: A review},
  author={Paul, Debashis and Aue, Alexander},
  journal={Journal of Statistical Planning and Inference},
  volume={150},
  pages={1--29},
  year={2014},
  publisher={Elsevier}
}

@article{yin1984limit,
  title={On limit of the largest eigenvalue of the large dimensional sample covariance matrix},
  author={Yin, YQ and Bai, ZD and Krishnaiah, PR},
  year={1984}
}

@incollection{bai2008limit,
  title={Limit of the smallest eigenvalue of a large dimensional sample covariance matrix},
  author={Bai, Zhi-Dong and Yin, Yong-Qua},
  booktitle={Advances In Statistics},
  pages={108--127},
  year={2008},
  publisher={World Scientific}
}

@article{johnstone2001distribution,
  title={On the distribution of the largest eigenvalue in principal components analysis},
  author={Johnstone, Iain M},
  journal={The Annals of statistics},
  volume={29},
  number={2},
  pages={295--327},
  year={2001},
  publisher={Institute of Mathematical Statistics}
}

@article{tracy1996orthogonal,
  title={On orthogonal and symplectic matrix ensembles},
  author={Tracy, Craig A and Widom, Harold},
  journal={Communications in Mathematical Physics},
  volume={177},
  pages={727--754},
  year={1996},
  publisher={Springer}
}

@article{karoui2003largest,
  title={On the largest eigenvalue of Wishart matrices with identity covariance when n, p and p/n tend to infinity},
  author={Karoui, Noureddine El},
  journal={arXiv preprint math/0309355},
  year={2003}
}


@article{wachter1980limiting,
  title={The limiting empirical measure of multiple discriminant ratios},
  author={Wachter, Kenneth W},
  journal={The Annals of Statistics},
  pages={937--957},
  year={1980},
  publisher={JSTOR}
}

@article{yin1983limit,
  title={A limit theorem for the eigenvalues of product of two random matrices},
  author={Yin, Yong Q and Krishnaiah, Paruchuri R},
  journal={Journal of Multivariate Analysis},
  volume={13},
  number={4},
  pages={489--507},
  year={1983},
  publisher={Elsevier}
}

@article{yin1986limiting,
  title={Limiting spectral distribution for a class of random matrices},
  author={Yin, Yong Q},
  journal={Journal of multivariate analysis},
  volume={20},
  number={1},
  pages={50--68},
  year={1986},
  publisher={Elsevier}
}

@article{yin1983limiting,
  title={Limiting behavior of the eigenvalues of a multivariate F matrix},
  author={Yin, YQ and Bai, ZD and Krishnaiah, PR},
  journal={Journal of multivariate analysis},
  volume={13},
  number={4},
  pages={508--516},
  year={1983},
  publisher={Elsevier}
}

@article{bai1988limiting,
  title={On the limiting empirical distribution function of the eigenvalues of a multivariate F matrix},
  author={Bai, Zhidong D and Yin, Yong Q and Krishnaiah, Paruchuri R},
  journal={Theory of Probability \& Its Applications},
  volume={32},
  number={3},
  pages={490--500},
  year={1988},
  publisher={SIAM}
}

@article{han2016tracy,
  title={The Tracy--Widom law for the largest eigenvalue of F type matrices},
  author={Han, Xiao and Pan, Guangming and Zhang, Bo},
  year={2016}
}


@article{ryan2023detecting,
  title={Detecting changes in covariance via random matrix theory},
  author={Ryan, Sean and Killick, Rebecca},
  journal={Technometrics},
  volume={65},
  number={4},
  pages={480--491},
  year={2023},
  publisher={Taylor \& Francis}
}

@article{bhattacharjee2016large,
  title={Large sample behaviour of high dimensional autocovariance matrices},
  author={Bhattacharjee, Monika and Bose, Arup},
  year={2016}
}

@book{bai2010spectral,
  title={Spectral analysis of large dimensional random matrices},
  author={Bai, Zhidong and Silverstein, Jack W},
  volume={20},
  year={2010},
  publisher={Springer}
}

@article{johnstone2006high,
  title={High dimensional statistical inference and random matrices},
  author={Johnstone, Iain M},
  journal={arXiv preprint math/0611589},
  year={2006}
}


@book{couillet2011random,
  title={Random matrix methods for wireless communications},
  author={Couillet, Romain and Debbah, Merouane},
  year={2011},
  publisher={Cambridge University Press}
}

@article{bai2007signal,
  title={On the signal-to-interference ratio of CDMA systems in wireless communications},
  author={Bai, ZD and Silverstein, Jack W},
  year={2007}
}

@article{nadakuditi2010fundamental,
  title={Fundamental limit of sample generalized eigenvalue based detection of signals in noise using relatively few signal-bearing and noise-only samples},
  author={Nadakuditi, Raj Rao and Silverstein, Jack W},
  journal={IEEE Journal of selected topics in Signal Processing},
  volume={4},
  number={3},
  pages={468--480},
  year={2010},
  publisher={IEEE}
}

@article{silverstein1992signal,
  title={Signal detection via spectral theory of large dimensional random matrices},
  author={Silverstein, Jack W and Combettes, Patrick L},
  journal={IEEE Transactions on Signal Processing},
  volume={40},
  number={8},
  pages={2100--2105},
  year={1992},
  publisher={IEEE}
}

@article{hachem2013subspace,
  title={A subspace estimator for fixed rank perturbations of large random matrices},
  author={Hachem, Walid and Loubaton, Philippe and Mestre, Xavier and Najim, Jamal and Vallet, Pascal},
  journal={Journal of Multivariate Analysis},
  volume={114},
  pages={427--447},
  year={2013},
  publisher={Elsevier}
}

@article{roy1953heuristic,
  title={On a heuristic method of test construction and its use in multivariate analysis},
  author={Roy, Samarendra Nath},
  journal={The Annals of Mathematical Statistics},
  volume={24},
  number={2},
  pages={220--238},
  year={1953},
  publisher={Institute of Mathematical Statistics}
}

@article{johnstone2017roy,
  title={Roy’s largest root test under rank-one alternatives},
  author={Johnstone, Iain M and Nadler, Boaz},
  journal={Biometrika},
  volume={104},
  number={1},
  pages={181--193},
  year={2017},
  publisher={Oxford University Press}
}

@article{kritchman2009non,
  title={Non-parametric detection of the number of signals: Hypothesis testing and random matrix theory},
  author={Kritchman, Shira and Nadler, Boaz},
  journal={IEEE Transactions on Signal Processing},
  volume={57},
  number={10},
  pages={3930--3941},
  year={2009},
  publisher={IEEE}
}


@article{niu2016multiple,
  title={Multiple change-point detection: a selective overview},
  author={Niu, Yue S and Hao, Ning and Zhang, Heping},
  journal={Statistical Science},
  pages={611--623},
  year={2016},
  publisher={JSTOR}
}

@article{aminikhanghahi2017survey,
  title={A survey of methods for time series change point detection},
  author={Aminikhanghahi, Samaneh and Cook, Diane J},
  journal={Knowledge and information systems},
  volume={51},
  number={2},
  pages={339--367},
  year={2017},
  publisher={Springer}
}


@inproceedings{banerjee2015non,
  title={Non-parametric quickest change detection for large scale random matrices},
  author={Banerjee, Taposh and Firouzi, Hamed and Hero, Alfred O},
  booktitle={2015 IEEE International Symposium on Information Theory (ISIT)},
  pages={146--150},
  year={2015},
  organization={IEEE}
}

@article{hero2012hub,
  title={Hub discovery in partial correlation graphs},
  author={Hero, Alfred and Rajaratnam, Bala},
  journal={IEEE Transactions on Information Theory},
  volume={58},
  number={9},
  pages={6064--6078},
  year={2012},
  publisher={IEEE}
}

@article{avanesov2018change,
  title={Change-point detection in high-dimensional covariance structure},
  author={Avanesov, Valeriy and Buzun, Nazar},
  year={2018}
}

@article{wang2017optimal,
  title={Optimal covariance change point localization in high dimension},
  author={Wang, Daren and Yu, Yi and Rinaldo, Alessandro},
  journal={arXiv preprint arXiv:1712.09912},
  year={2017}
}

@article{bhattacharjee2016large,
  title={Large sample behaviour of high dimensional autocovariance matrices},
  author={Bhattacharjee, Monika and Bose, Arup},
  year={2016}
}

@book{finn1974general,
  title={A general model for multivariate analysis.},
  author={Finn, Jeremy D},
  year={1974},
  publisher={Holt, Rinehart \& Winston}
}

@article{wilks1932certain,
  title={Certain generalizations in the analysis of variance},
  author={Wilks, Samuel S},
  journal={Biometrika},
  pages={471--494},
  year={1932},
  publisher={JSTOR}
}

@article{lawley1938generalization,
  title={A generalization of Fisher's z test},
  author={Lawley, Derrick N},
  journal={Biometrika},
  volume={30},
  number={1/2},
  pages={180--187},
  year={1938},
  publisher={JSTOR}
}

@article{potthoff1964generalized,
  title={A generalized multivariate analysis of variance model useful especially for growth curve problems},
  author={Potthoff, Richard F and Roy, Samarendra N},
  journal={Biometrika},
  volume={51},
  number={3-4},
  pages={313--326},
  year={1964},
  publisher={Oxford University Press}
}

@article{haynes2013bonferroni,
  title={Bonferroni correction},
  author={Haynes, Winston},
  journal={Encyclopedia of systems biology},
  pages={154--154},
  year={2013},
  publisher={Springer New York}
}

@article{scott1974cluster,
  title={A cluster analysis method for grouping means in the analysis of variance},
  author={Scott, Andrew Jhon and Knott, Martin},
  journal={Biometrics},
  pages={507--512},
  year={1974},
  publisher={JSTOR}
}

@article{olshen2004circular,
  title={Circular binary segmentation for the analysis of array-based DNA copy number data},
  author={Olshen, Adam B and Venkatraman, E Seshan and Lucito, Robert and Wigler, Michael},
  journal={Biostatistics},
  volume={5},
  number={4},
  pages={557--572},
  year={2004},
  publisher={Oxford University Press}
}

@article{fryzlewicz2014wild,
  title={Wild binary segmentation for multiple change-point detection},
  author={Fryzlewicz, Piotr},
  year={2014}
}

@article{ma2012accuracy,
  title={Accuracy of the Tracy--Widom limits for the extreme eigenvalues in white Wishart matrices},
  author={Ma, Zongming},
  year={2012}
}

@article{soshnikov2002note,
  title={A note on universality of the distribution of the largest eigenvalues in certain sample covariance matrices},
  author={Soshnikov, Alexander},
  journal={Journal of Statistical Physics},
  volume={108},
  pages={1033--1056},
  year={2002},
  publisher={Springer}
}

@article{hastie1995penalized,
  title={Penalized discriminant analysis},
  author={Hastie, Trevor and Buja, Andreas and Tibshirani, Robert},
  journal={The Annals of Statistics},
  volume={23},
  number={1},
  pages={73--102},
  year={1995},
  publisher={Institute of Mathematical Statistics}
}

@article{telatar1999capacity,
  title={Capacity of multi-antenna Gaussian channels},
  author={Telatar, Emre},
  journal={European transactions on telecommunications},
  volume={10},
  number={6},
  pages={585--595},
  year={1999},
  publisher={Wiley Online Library}
}

@article{hoyle2003limiting,
  title={Limiting form of the sample covariance eigenspectrum in PCA and kernel PCA},
  author={Hoyle, David and Rattray, Magnus},
  journal={Advances in Neural Information Processing Systems},
  volume={16},
  year={2003}
}

@article{johnstone2009sparse,
  title={Sparse principal components analysis},
  author={Johnstone, Iain M and Lu, Arthur Yu},
  journal={arXiv preprint arXiv:0901.4392},
  year={2009}
}

@article{baik2006eigenvalues,
  title={Eigenvalues of large sample covariance matrices of spiked population models},
  author={Baik, Jinho and Silverstein, Jack W},
  journal={Journal of multivariate analysis},
  volume={97},
  number={6},
  pages={1382--1408},
  year={2006},
  publisher={Elsevier}
}

@article{paul2007asymptotics,
  title={Asymptotics of sample eigenstructure for a large dimensional spiked covariance model},
  author={Paul, Debashis},
  journal={Statistica Sinica},
  pages={1617--1642},
  year={2007},
  publisher={JSTOR}
}

@article{bai2008large,
  title={Large sample covariance matrices without independence structures in columns},
  author={Bai, Zhidong and Zhou, Wang},
  journal={Statistica Sinica},
  pages={425--442},
  year={2008},
  publisher={JSTOR}
}

@article{pinelis2016optimal,
  title={Optimal-order bounds on the rate of convergence to normality in the multivariate delta method},
  author={Pinelis, Iosif and Molzon, Raymond},
  year={2016}
}

@article{olkin1964multivariate,
  title={Multivariate beta distributions and independence properties of the Wishart distribution},
  author={Olkin, Ingram and Rubin, Herman},
  journal={The Annals of Mathematical Statistics},
  pages={261--269},
  year={1964},
  publisher={JSTOR}
}

@article{perlman1977note,
  title={A note on the matrix-variate F distribution},
  author={Perlman, Michael D},
  journal={Sankhy{\=a}: The Indian Journal of Statistics, Series A},
  pages={290--298},
  year={1977},
  publisher={JSTOR}
}

@article{wax1985detection,
  title={Detection of signals by information theoretic criteria},
  author={Wax, Mati and Kailath, Thomas},
  journal={IEEE Transactions on acoustics, speech, and signal processing},
  volume={33},
  number={2},
  pages={387--392},
  year={1985},
  publisher={IEEE}
}

@article{anderson1963asymptotic,
  title={Asymptotic theory for principal component analysis},
  author={Anderson, Theodore Wilbur},
  journal={The Annals of Mathematical Statistics},
  volume={34},
  number={1},
  pages={122--148},
  year={1963},
  publisher={Institute of Mathematical Statistics}
}


@article{pearson1901liii,
  title={LIII. On lines and planes of closest fit to systems of points in space},
  author={Pearson, Karl},
  journal={The London, Edinburgh, and Dublin philosophical magazine and journal of science},
  volume={2},
  number={11},
  pages={559--572},
  year={1901},
  publisher={Taylor \& Francis}
}

@article{johnson1972analysis,
  title={An analysis of a two-way model with interaction and no replication},
  author={Johnson, Dallas E and Graybill, Franklin A},
  journal={Journal of the American Statistical Association},
  volume={67},
  number={340},
  pages={862--868},
  year={1972},
  publisher={Taylor \& Francis}
}

@article{nadler2008finite,
  title={Finite sample approximation results for principal component analysis: A matrix perturbation approach},
  author={Nadler, Boaz},
  year={2008}
}

@article{tipping1999probabilistic,
  title={Probabilistic principal component analysis},
  author={Tipping, Michael E and Bishop, Christopher M},
  journal={Journal of the Royal Statistical Society Series B: Statistical Methodology},
  volume={61},
  number={3},
  pages={611--622},
  year={1999},
  publisher={Oxford University Press}
}

@article{forni2000tthe,
  title={TThe generalized factor model: identification and estimation},
  author={Forni, M and Hallin, M and Lippi, M and Reichlin, L},
  journal={U\%"" 3\&},
  volume={4},
  year={2000}
}


@article{deb2017asymptotic,
  title={An asymptotic theory for spectral analysis of random fields},
  author={Deb, Soudeep and Pourahmadi, Mohsen and Wu, Wei Biao},
  year={2017}
}


